CLD -- A Detector Concept for the FCC-ee

This note gives a conceptual description and illustration of the CLD detector, based on the work for a detector at CLIC. CLD is one of the detectors envisaged at a future 100 km $e^+e^-$ circular collider (FCC-ee). The note also contains a brief description of the simulation and reconstruction tools used in the linear collider community, which have been adapted for physics and performance studies of CLD. The detector performance is described in terms of single particles, particles in jets, jet energy and angular resolution, and flavour tagging. The impact of beam-related backgrounds (incoherent $e^+e^-$ pairs and synchrotron radiation photons) on the performance is also discussed.

==> include/flavour_tagging.tex <==




\clearpage

\subsection{Flavour_Tagging}
\label{subsec:flavourtag}

 FIXME - this is just copied from the CLICdet performance note, needs to be modified !

Flavour tagging studies were performed initially in the CDR~\cite{cdrvol2} (section 12.3.4) for the \clicsid detector model. 
These studies were extended to explore more realistic vertex detector geometries~\cite{Alipour_Roloff_2014}, 
e.g.\ using spirals instead of forward disks, thus allowing for air flow cooling of the vertex detector system.
One of the main findings of~\cite{Alipour_Roloff_2014} is related to the material budget: Doubling the material per layer in the vertex detector
(as required for the more realistic design adapted for CLICdet) leads to a degradation of the flavour tagging performance. The fake rates
are found to deteriorate by 5\% to 35\%.


The vertex detector geometry of CLICdet has recently been used for additional studies, using the software chain described in section~\ref{sec:simreco} and the flavour tagging package LCFIPlus~\cite{suehara:2015ura}. 
Complementing the exploratory studies of~\cite{Alipour_Roloff_2014}, as a first step the dependence of performance on the assumed single point resolution in the vertex detector layers was investigated in $\epem\to\bb$ 
events at 500 GeV\@. The primary vertex position resolution for a single point resolution of 3, 5 and 7~\micron is shown in Figures~\ref{fig:pvx_res} and~\ref{fig:pvz_res}. 
As expected, the vertex resolution improves approximately with 1/N (N is the number of tracks). The secondary vertex position resolution obtained from LCFIPlus is shown in Figures~\ref{fig:svx_res} and~\ref{fig:svz_res}.
 Both primary and secondary vertex z-resolution show the anticipated strong dependence on the angle $\theta$ of the tracks.

\begin{figure}[bp]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{vs N}
  \label{fig:pvxresN}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
   \caption{vs $\theta$}
  \label{fig:pvsresTheta}
\end{subfigure}
\caption{Primary vertex x-resolution as a function of number of tracks (a) and polar angle (b), for three  different assumptions on the single point resolution. Note that the y-resolution is found to be identical.}
\label{fig:pvx_res}
\end{figure}



\begin{figure}[htbp]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{vs N}
  \label{fig:pvzresN}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
   \caption{vs $\theta$}
  \label{fig:pvzresTheta}
\end{subfigure}
\caption{Primary vertex z-resolution as a function of number of tracks (a) and polar angle (b), for three  different assumptions on the single point resolution.}
\label{fig:pvz_res}
\end{figure}

\begin{figure}[htbp]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{vs N}
  \label{fig:svxresN}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
   \caption{vs $\theta$}
  \label{fig:svxresTheta}
\end{subfigure}
\caption{Secondary vertex x-resolution as a function of number of tracks (a) and polar angle $\theta$ (b), where  $\theta$ here denotes the angle of particles associated to the secondary vertex, 
for three different assumptions on the single point resolution. The y-resolution is found to be identical.}
\label{fig:svx_res}
\end{figure}

 
\begin{figure}[htbp]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{vs N}
  \label{fig:svzresN}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
   \caption{vs $\theta$}
  \label{fig:svzresTheta}
\end{subfigure}
\caption{Secondary vertex z-resolution as a function of number of tracks (a) and polar angle $\theta$ (b), where $\theta$ here denotes the angle of particles associated to the secondary vertex, for three different assumptions on the single point resolution.}
\label{fig:svz_res}
\end{figure}

The combined impact on flavour tagging performance, when worsening the single point resolution from the nominal 3~\micron{} to 5 or 7~\micron, 
was then investigated using dijet samples at 500~GeV\@. Figure~\ref{fig:flavourtag_beauty_vs_singlepoint} shows the results obtained for beauty tagging, 
where the misidentification probability for charm and light flavour quark background is shown as a function of b-tagging efficiency. As expected,
 the results get worse for the less performant vertexing - the hypothetical position resolution of 1~\micron is shown for reference. The variation is comparable for the cases of charm and light-flavour background. Similarly, charm tagging has been investigated and it is shown in Figure~\ref{fig:flavourtag_charm_vs_singlepoint}. The variation appears to be stronger for the case of light-flavour background than for the case of charm background. In general, c-tagging is more strongly dependent on single point resolution than b-tagging.

\begin{figure}[tbp]
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
         \caption{Performance  of beauty tagging for different assumptions on the single point resolution in the vertex detector. The misidentification probability is given on the left for charm background, on the right for light flavour background.}
   \label{fig:flavourtag_beauty_vs_singlepoint}
\end{figure}
\begin{figure}[tbp]
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
         \caption{Performance  of charm tagging for different assumptions on the single point resolution in the vertex detector. The misidentification probability is given on the left for beauty background, on the right for light flavour background.}
   \label{fig:flavourtag_charm_vs_singlepoint}
\end{figure}

The overall performance of flavour tagging at CLICdet has been tested using the nominal parameters (e.g. 3~\micron{} position resolution), 
and comparing the beauty and charm tagging results without and with overlay of \gghad{} background corresponding to 30 bunch crossings. 
Figure~\ref{fig:beff_ceff_background} shows the results obtained. The b-tagging performance is typically worse by about 20\%--30\%, while the c-tagging performance seems to be less degraded due the \gghad{} background, at the level of about 15\%.

\begin{figure}[tbp]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{beauty}
  \label{fig:b_mis_eff}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
   \caption{charm}
  \label{fig:c_mis_eff}
\end{subfigure}
\caption{Global performance  of beauty tagging (a) and charm tagging (b) for jets in dijet events at $\roots = 500~\mathrm{GeV}$
with a mixture of polar angles between 20\degrees{} and 90\degrees{}. A comparison of performance with and without \gghad{} background is presented. On the y-axis,
the misidentification probability and the ratio of the misidentification probabilities with and without \gghad{} background are given.}
\label{fig:beff_ceff_background}
\end{figure}

Comparing the result obtained presently for CLICdet (Figure~\ref{fig:beff_ceff_background}) with the earlier results using a similar vertex detector layout and material budget~\cite{Alipour_Roloff_2014}, one finds that the
performance for b-tagging in CLICdet is worse. On the other hand, the performance for c-tagging is considerably improved in CLICdet. In order to investigate the possible cause for the deficiencies in b-tagging performance,
the default ConformalTracking in the software chain was replaced by TruthTracking (see \cref{sec:event-reconstruction}).

The comparison of flavour tagging with TruthTracking and ConformalTracking, shown in Figure~\ref{fig:beff_ceff_TTCT}, indicates indeed that further improvements in the ConformalTracking algorithm are necessary to enhance the flavour tagging capabilities of CLICdet.  

\begin{figure}[htbp]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{beauty}
  \label{fig:b_eff_TTCT}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
   \caption{charm}
  \label{fig:c_eff_TTCT}
\end{subfigure}
\caption{Performances of beauty tagging (a) and charm tagging (b) for jets in dijet events at $\roots = 500\mathrm{GeV}$
with a mixture of polar angles between 20\degrees{} and 90\degrees{}. A comparison of performance using TruthTracking with respect to ConformalTracking is shown. On the y-axis, the misidentification probability and the ratio of the misidentification probabilities with and without \gghad{} background are given.}
\label{fig:beff_ceff_TTCT}
\end{figure}

In this respect, particularly enlightening is the comparison of the two-dimensional radial distributions of secondary vertices for beauty, charm and light quark events, shown in Figures~\ref{fig:SVvsR_bb_cc} and~\ref{fig:SVvsR_qq}. 
Two features emerge from these plots: a) a consistent drop off for TruthTracking at a radius of 50~mm and b) an excess of secondary vertices for ConformalTracking.
The former feature comes from the selection of tracks used by the particle flow reconstruction for creating links between clusters and tracks. 
Tracks with a first hit beyond 50~mm radius are not used for creating \emph{particle flow objects} and will therefore also not be used in the vertexing. 
Although this cut-off is applied in the same way for the ConformalTracking, the effect is reduced due to issues in the pattern recognition, 
which are also at the origin of the second feature. Here the problem is represented by clones and split tracks, absent in TruthTracking.
Clones are defined as tracks that share two or more hits. Split tracks occur when a Monte Carlo particle is reconstructed as two (or more) tracks.
Two cases have been observed: a) these tracks are spatially separated, e.g.\ one is reconstructed with hits from the vertex detector and other one with hits from the tracker detector;
 b) the particles hits are split between the tracks along the full particle length.
Both clones and split tracks are able to mimic the existence of secondary vertices, thus causing the difference between TruthTracking and ConformalTracking.
Future improvements in the track and particle flow reconstruction to solve the overall discrepancies are described in \cref{sec:FutureImp}.


\begin{figure}[htbp]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{\bb{}}
  \label{fig:SVvsR_bb}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
   \caption{\cc{}}
  \label{fig:SVvsR_cc}
\end{subfigure}
\caption{Secondary vertex radius distribution for \bb{} (a) and \cc{} (b) events, comparing TruthTracking and ConformalTracking.}
\label{fig:SVvsR_bb_cc}
\end{figure}

\begin{figure}[htbp]
  \centering
\missingfigure[figwidth=7.0cm]{waiting for image}
  \caption{Secondary vertex radius distribution for events of dijets from light quarks, comparing TruthTracking and ConformalTracking.}
   \label{fig:SVvsR_qq}
\end{figure}





==> vertex.tex <==


 


\clearpage


\section{Vertex Detector}
\label{vertex}
\subsection{Overview and Layout}
The vertex detector in the CLD concept, a scaled version of the one in CLICdet, consists of a cylindrical barrel detector closed off in the forward directions by discs.
The layout is based on double layers, i.e. two sensitive layers fixed on a common support structure (which includes cooling circuits).
The barrel consists of three double layers, the forward region is covered by three sets of double-discs on both sides of the barrel. 
An overview of the vertex detector layout is given in Figure~\ref{fig.vertex.sketch}. The total area of the vertex detector sensors is 0.53~m$^2$.

\begin{figure}[hbtp] 
      \centering
            \includegraphics[scale=0.95]{./figures/full_VTX_FCCee_v2.pdf}
       \caption{ Sketch of the vertex detector  barrel and forward region (in the ZR plane) of the CLD simulation model. Dimensions are given in mm. 
Red lines indicate sensors, black lines support structure, while magenta lines show cables. The vacuum beam pipe is shown in orange colour.}
       \label{fig.vertex.sketch}
\end{figure}

The vertex detector consists of 25~$\times$~25~$\micron^2$  pixels, with a silicon sensor thickness of 50~\micron.
Using pulse height information and charge sharing, a single point resolution of 3~\micron is aimed for.

The inner radius of the innermost vertex barrel layer is determined by the radius and thickness of the central beam pipe, which in turn is given by MDI constraints~\cite{FCC_CDR}.
As a result, the inner edge of the  innermost layer of the vertex barrel is located at R~=~17.5~mm. The location of the additional vertex barrel layers is obtained by scaling-down the layout of the CLICdet vertex detector layout.

The overall length of the barrel vertex detector, built from staves, is 250~mm. 
The double layer structure is shown in Figure~\ref{fig:vertex.options}.
 Further details on the dimensions of the vertex detector
barrel layers used in the simulation model are given in Table~\ref{tab.vertex.geometry.for.tracking}. 
Note that the present numbers for the stave widths result from scaling-down the CLICdet layout -- these are the numbers implemented in the simulation model.
 In a forthcoming engineering study, such layout details will have to be revised.

\begin{figure}[hbtp]
         \centering
                \includegraphics[width=0.50\textwidth]{./figures/VTX_barrel_view.pdf}   
 \caption{The double layer arrangement in the vertex barrel detector (XY view).}
\label{fig:vertex.options}
\end{figure}


\begin{table}[b!]
   \centering
   \caption{Vertex barrel layout as implemented in the simulations.}
\label{tab.vertex.geometry.for.tracking}
   \begin{tabular}[h!]{c c c c}
\toprule
Barrel layers&	Inner radius [mm]   &  No. of staves & Stave width [mm]\\
\midrule
1 -- 2&17.5 -- 18.5 &  16&  7.3\\
3 -- 4&  37 -- 38&      12 &  20.2\\
5 -- 6&  57 -- 58 &   16  &    23.1\\
\bottomrule
   \end{tabular}
\end{table}
 
The vertex detector forward region consists of three discs on each side, each disc is built as a double-layer device.
The discs are located a distance from the IP of 160, 230 and 300~mm, respectively.
They are constructed from 8 trapezoids, approximating a circle. For simplicity the trapezoids are not overlapping in the simulation model. 
The inner radii of the forward discs respect the 150~mrad cone reserved for MDI elements.
The dimensions of the vertex forward discs are given in Table~\ref{tab.vertex.discs}.
Contrary to CLICdet, the forward region vertex detector is built from planar discs\footnote{The design with spirals in CLICdet is motivated by the optimisation of the air flow through the vertex region. 
Air cooling is deemed not to be sufficient for the CLD vertex detector.}.
An example of the vertex petal arrangement as implemented in the simulation is shown in Figure~\ref{fig.vertex.petals}. 


\begin{table}[hbtp]
   \centering
   \caption{Dimensions of the vertex discs.}
\label{tab.vertex.discs}
   \begin{tabular}[h!]{c c c c c}
\toprule
Vertex disc&	Inner radius [mm]   &  Outer radius [mm]\\
\midrule
1 & 24&  102\\
2&  34.5 &      102\\
3&  45  &   102\\
\bottomrule
   \end{tabular}
\end{table}

\begin{figure}[hbtp] 
      \centering
               \includegraphics[scale=0.6]{./figures/VTX_endcap_view.pdf}
       \caption{Schematic view of the first vertex forward disc, as implemented in the simulation model (XY view).}
       \label{fig.vertex.petals}
\end{figure}









\subsection{Beam-Induced Backgrounds in the Vertex Detector Region}
\label{vtx_background}


Beam-related backgrounds are significant drivers for the vertex and tracker technology choices and the requirements for the read-out of these detectors.
Three types of backgrounds have been studied in detail: incoherent \epem pair production and \gghad production from beam-beam interactions, and background hits from synchrotron 
radiation. The studies using full Monte Carlo simulations and their results are described in detail in section 7.1 of the CDR~\cite{FCC_CDR}.
Examples for incoherent pairs and synchrotron radiation at the lowest and highest energy of FCC-ee operation are given below. 
The rate of \gghad events was found to be negligible (< 0.008 events per bunch crossing at 365 GeV, <0.0007 per bunch crossing at 91.2 GeV).

The simulations were performed using the latest version of the CLD detector model and applying a realistic field map (resulting from the detector main solenoid field and the fields of the compensating and screening solenoids).
Figure~\ref{fig:VTX_pairs_91} shows the resulting hit density from incoherent pairs per bunch crossing (BX) for operation at the Z-pole, at 91.2 GeV, while Figure~\ref{fig:VTX_pairs_365} presents the same for the top energy, 365 GeV.
At 91.2 GeV, the result are obtained from simulating 1806 bunch crossings, while at 365 GeV sufficient statistical accuracy was obtained from 371 bunch crossings.
At 365 GeV, backscattering from forward region elements (such as LumiCal) appears to be dominant, leading to more hits at the extremities of the vertex detector barrel layers (Figure~\ref{fig:VTXB_pairs_365}). To the contrary, at 91.2 GeV direct hits (leading to more hits in the centre of the barrel) are dominant (Figure~\ref{fig:VTX_pairs_91}).

The corresponding results for hits related to synchrotron radiation photons (averaged over 10 bunch crossings) are shown 
in Figure~\ref{fig:VTX_sync_365}. These  hit rates are about a factor of five lower than the hits from incoherent pairs.
Note that there are no hits from synchrotron radiation observed at 91.2 GeV, even when accumulating data from more than 40000 bunch crossings.

From the hit densities obtained, one can deduce detector occupancies under certain assumptions, in analogy to what is described for CLICdet in~\cite{Nurnberg_Dannheim_2017}.

\begin{equation}
\begin{split}
Occupancy / (readout~window) = Hits / (mm^2 \cdot BX) \times n_{bunches} / (readout~window) \times \\[1em]
 \times (pixel~size) \times (avg.~cluster~size) \times (safety~factor)
\end{split}
\label{eq:occupancy}
\end{equation}

In the following, we are assuming a safety factor of 5 to account for uncertainties in the simulation, and a cluster size of 3 (which will depend on technology choices).
In a scenario where the technology chosen for the ALICE ITS LS2 upgrade~\cite{ALICE_ITS} is assumed, the readout time window\footnote{
Additional studies are required for the case of running at 91.2 GeV: the high rate of Z events (up to 100 kHz) might require some form of time stamping / time of arrival information within the readout window. 
On the other hand, given the rapid evolution of silicon pixel technology, a much shorter readout window with similar powering/cooling requirements is also conceivable.}. would be about 10 $\upmu{}$s.
The present FCC-ee design parameters foresee a bunch spacing of 19.6 ns at 91.2 GeV, and of 3396 ns at 365 GeV, leading to 510 and 3 bunch crossings, respectively,
within the readout window. As a result, the estimated maximal occupancies per readout window (including the safety factor) are expected to be 0.43\% and 0.13\% for operation at 91.2 and 365 GeV, respectively.
It is expected that such occupancies from background hits are acceptable and will not, e.g., impact the performance of the pattern recognition algorithm of the tracking software.


 



\begin{figure}[htbp]
  \centering
  \begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{./figures/VXDB_Z_CDR.pdf}
    \caption{}
    \label{fig:VTXB_pairs_91}
  \end{subfigure}%
  \begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{./figures/VXDE_Z_CDR.eps}
    \caption{}
    \label{fig:VTXE_Pairs_91}
  \end{subfigure}
  \caption{Hit densities per bunch crossing in the CLD vertex detector barrel layers (a) and  forward discs (b) for particles originating from incoherent pairs. 
Results are shown for operation at 91.2 GeV. VXD L1-L6 indicates the vertex detector barrel layers, while VXDE D1-D6 stands for the vertex detector forward discs.
Vertical error bars indicate the statistical uncertainty, horizontal bars are drawn to show the bin size.
Safety factors for the simulation uncertainties are not included. }
  \label{fig:VTX_pairs_91}
\end{figure}

\begin{figure}[htbp]
  \centering
  \begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{./figures/VXDB_365_CDR.pdf}
    \caption{}
    \label{fig:VTXB_pairs_365}
  \end{subfigure}%
  \begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{./figures/VXDE_365_CDR.eps}
    \caption{}
    \label{fig:VTXE_Pairs_365}
  \end{subfigure}
  \caption{Hit densities per bunch crossing in the CLD vertex detector barrel layers (a) and  forward discs (b) for particles originating from incoherent \epem pairs, for operation at 365 GeV. 
Vertical error bars indicate the statistical uncertainty, horizontal bars are drawn to show the bin size. Safety factors for the simulation uncertainties are not included. }
  \label{fig:VTX_pairs_365}
\end{figure}

\begin{figure}[htbp]
  \centering
  \begin{subfigure}{.5\textwidth}
    \centering
   \includegraphics[width=\linewidth]{./figures/VTDB_10BX.pdf}
    \caption{}
    \label{fig:VTXB_sync_365}
  \end{subfigure}%
  \begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=\linewidth]{./figures/VTDE_10BX.pdf}
    \caption{}
    \label{fig:VTXE_sync_365}
  \end{subfigure}
  \caption{As Figure~\ref{fig:VTX_pairs_365} but for hits related to synchrotron radiation photons. }
  \label{fig:VTX_sync_365}
\end{figure}





 

\subsection{Technology Choices, Cooling and Material Budget}
\label{vtx_technology}

The technologies available for vertex pixel sensors, readout electronics, mechanical support structures, and cooling are rapidly evolving. At this stage of the conceptual design for CLD,
the example of the ALICE ITS LS2 upgrade~\cite{ALICE_ITS} is considered an acceptable approximation for the amount of material, to be used in the simulation model.

The ALICE ITS upgrade uses very light-weight structures. The average power dissipation is measured in prototypes to be about 40~mW/cm${^2}$, and water cooling is used for the devices.
Assuming this technology, the total material budget per double layer in the CLD vertex detector is 0.6\%~\radlen. For reference, this corresponds to 50\% more material than in the CLICdet vertex detector
which assumes power pulsing and air cooling.

The low occupancies expected from incoherent pairs and synchrotron radiation (see Section~\ref{vtx_background}), at all energy stages of FCC-ee,
allow one to overlay events from a large number of bunch crossings -- this implies that rather long readout integration times are acceptable for the CLD vertex detector.

A simplified vertex layer layout is implemented in the simulation model. The 50~\micron silicon sensors are separated by a 1~mm air-gap in the barrel and a  2~mm air-gap in the discs. 
On the outside of each sensor, additional material represented by 235~\micron of silicon replaces the combined material of ASIC, support structure, connectivity and cooling. 
The resulting total material budget per double layer corresponds to the thickness in \radlen expected to emerge from the engineering design (and has been achieved in the ALICE ITS upgrade). A summary is given in Table~\ref{table:vertex_material}.
Note that, in analogy to CLICdet, slightly more material is assumed to be needed for the mechanical support of the vertex discs w.r.t. the barrel layers, resulting in a total material budget of 0.7\%~\radlen for the discs.


\begin{table}[h!]
   \centering
   \caption{Vertex detector double layer material budget as implemented in the simulations.}
\label{table:vertex_material}
   \begin{tabular}[h!]{c c c c c c}
\toprule
       Function &Material  & \multicolumn{2}{c}{Barrel} & \multicolumn{2}{c}{Discs} \\
       \cmidrule(lr){3-4} \cmidrule(l){5-6}
&	  &  Thickness  & Material budget & Thickness & Material budget \\
       &	  &  [\micron{}] &  \radlen~[\%{}] &  [\micron{}] &   \radlen~[\%{}] \\
\midrule
ASIC, support etc.& Silicon  &   235 &  0.259& 280& 0.298\\
Sensor& Silicon &  50&  0.053 & 50&  0.053 \\
Gap&  Air  &   1000  &   0.001 &2000 &0.001\\
Sensor& Silicon &  50&  0.053 & 50&  0.053 \\
ASIC, support etc.& Silicon  &   235 &  0.259& 280& 0.298\\
\midrule
total & & &0.625 & &0.703 \\
\bottomrule
   \end{tabular}
\end{table}





